Sakshm AI: Advancing AI-Assisted Coding Education for Engineering Students in India Through Socratic Tutoring and Comprehensive Feedback

The advent of Large Language Models (LLMs) is reshaping education, particularly in programming, by enhancing problem-solving, enabling personalized feedback, and supporting adaptive learning. Existing AI tools for programming education struggle with key challenges, including the lack of Socratic guidance, direct code generation, limited context retention, minimal adaptive feedback, and the need for prompt engineering. To address these challenges, we introduce Sakshm AI, an intelligent tutoring system for learners across all education levels. It fosters Socratic learning through Disha, its inbuilt AI chatbot, which provides context-aware hints, structured feedback, and adaptive guidance while maintaining conversational memory and supporting language flexibility. This study examines 1170 registered participants, analyzing platform logs, engagement trends, and problem-solving behavior to assess Sakshm AI's impact. Additionally, a structured survey with 45 active users and 25 in-depth interviews was conducted, using thematic encoding to extract qualitative insights. Our findings reveal how AI-driven Socratic guidance influences problem-solving behaviors and engagement, offering key recommendations for optimizing AI-based coding platforms. This research combines quantitative and qualitative insights to inform AI-assisted education, providing a framework for scalable, intelligent tutoring systems that improve learning outcomes. Furthermore, Sakshm AI represents a significant step toward Sustainable Development Goal 4 Quality Education, providing an accessible and structured learning tool for undergraduate students, even without expert guidance. This is one of the first large-scale studies examining AI-assisted programming education across multiple institutions and demographics.

==> files/05-evaluation.tex <==
% \subsection{ Quantitative analysis }





% \subsection{ Qualitative analysis }

% \subsubsection{\textbf{User Engagement and Platform Utilization}}\hfill\\

% The Sakshm platform has garnered significant engagement from students due to its innovative AI-driven features, particularly the AI chatbot, Disha, which provides personalized feedback, maintains code context, and encourages problem-solving through hints rather than direct solutions. Users leverage the platform for coding practice, tackling Data Structures and Algorithms (DSA) challenges, and preparing for interviews with questions tailored to specific companies like Flipkart, Accenture, Amazon, and Google. Its well-organized structure, customizable learning paths, and a wide variety of question sheets are highly appreciated, fostering an environment where learners can easily follow along, choose their learning path, and engage with coding exercises that are directly relevant to real-world applications.

% Students have shown a diverse preference for coding practice platforms, often leveraging multiple tools to meet various learning and interview preparation needs. LeetCode stands out as a favorite due to its vast repository of interview-style questions from leading companies, its user-friendly interface, and its popularity among the coding community. However, for those seeking alternatives or additional resources, GeeksforGeeks serves as a valuable supplement, particularly when LeetCode's premium features are out of reach. InterviewBit is also appreciated for its interview-focused questions, offering a different perspective on problem-solving. In terms of visual learning preferences, there is a clear inclination towards platforms that offer visual aids like videos or diagrams, with users expressing that such content not only aids comprehension but also keeps them engaged. The integration of AI tools like ChatGPT for debugging and learning concepts is also notable, indicating a shift towards more interactive and immediate learning support. Moreover, platforms like Coursera and Udemy are used for structured learning paths, providing a comprehensive approach to coding education. Users also mention the need for features like dark mode to enhance the coding experience, reflecting a desire for comfort during extended coding sessions. This variety in platform usage and learning preferences underscores the importance of having multiple resources available to cater to different learning styles and objectives.

% However, there exists a spectrum of opinions regarding the platform's accessibility and personalization. While many users find the AI's guidance valuable, some express a need for more tailored interactions to match individual learning styles or pace. This indicates a potential area for improvement, particularly in addressing occasional internet issues or enhancing the one-on-one interaction experience to make the platform even more user-friendly and effective. Users also appreciate the platform's focus on data structures and the ability to practice topic-wise, which is seen as particularly helpful for those still learning the basics. The platform's practice-oriented approach, where Disha prompts users to think through problems independently, is widely recognized for fostering a deeper understanding and confidence in coding. Additionally, Sakshm's unique features like the consolidated interface, where everything from code to test cases is available on a single screen, contribute to its user-friendly nature, although some users suggest improvements in interface simplicity and responsiveness.

% \emph{\textbf{"I like the layout of the courses. Everything is organized in a way that makes it easy to follow along."-[P1]}}

% \emph{\textbf{"Sakshm is the only platform with an AI chatbot," highlighting its uniqueness in fostering a more interactive learning environment-[P15]}}


% \subsubsection{\textbf{Effectiveness in Learning and Problem-Solving}}\hfill\\
% Sakshm's effectiveness in promoting independent thinking and problem-solving skills is widely acknowledged. The platform's method of providing hints rather than direct answers encourages users to think critically and solve problems independently, which many find beneficial. However, there are differing views on its efficacy across all difficulty levels. Users appreciate the step-by-step guidance for complex problems, but some need more direct support or additional resources for extremely challenging tasks. The AI's role in guiding thought processes rather than just giving answers is generally well-received, although there is a desire for the platform to incorporate more real-world examples and advanced topics to bridge the gap between beginner and intermediate levels.

% \emph{\textbf{"I think the copying approach is not there in Disha but rather in other AI platforms where I can just copy things. Disha is more intuitive, thought-provoking, and helpful."-[P1]}}

% \emph{\textbf{"I’ve improved at solving medium-level Python questions, though I still find data structures challenging."-[P6]}}

% \subsubsection{\textbf{Challenges and Suggestions for Improvement}}\hfill\\

% Users of the Sakshm platform have identified multiple areas for enhancement to enrich their learning experience. One of the primary concerns is the need for greater variety in coding exercises, with a particular call for more real-world problem-solving scenarios and the inclusion of additional programming languages to cater to a broader audience. This would not only make the platform more engaging but also better prepare students for the complexities of modern coding challenges, which often require the application of multiple concepts simultaneously. Moreover, users suggest that the AI, Disha, could improve its responsiveness, especially in providing immediate feedback after code submission, to enhance user interaction and reduce frustration during practice sessions.

% Regarding the AI's guidance, users feel that while the Socratic method promotes independent thinking, it could be more straightforward for simpler queries or under time constraints. They recommend incorporating common mistakes into the AI's training model to simulate a more teacher-like interaction, providing a balance between guiding thought processes and offering practical solutions when necessary. The platform's interface has also come under scrutiny, with users noting occasional lagginess, especially when navigating between topics or questions. Suggestions include improving server speed, enhancing the UI for smoother navigation, and reducing clutter to make coding sessions more efficient.

% Additionally, users express a desire for more detailed and personalized feedback. The platform should evaluate a student's progress more comprehensively, providing hints initially, then offering snippets or sub-solutions when needed, similar to an in-person tutor. This would address the frustration of dealing with abstract or overly vague responses, which can sometimes lead users to seek external resources for clarity. Another aspect mentioned is the integration of real interview experiences from alumni who have used the platform for preparation, which could provide insights into what companies look for and how to approach interview questions.

% \emph{\textbf{"There could be more variety in the exercises, and it should have more questions."-[P1]}}

% \emph{\textbf{"Disha could be a bit faster and more accurate with replies," pointing towards improvements in user interaction-[P17]}}

% \subsubsection{\textbf{Impact of AI on Problem-Solving and Learning}}\hfill\\

% The impact of AI on problem-solving and learning through Sakshm is viewed positively by many, with AI tools like Disha facilitating learning by guiding thought processes and offering immediate assistance for doubt resolution. However, there is a nuanced perspective on how AI tools might affect independent thinking. Some users appreciate the AI for reducing reliance on external resources and encouraging problem-solving, while others express concerns about over-reliance potentially diminishing their critical thinking abilities. Users also highlight the balance between convenience and growth, indicating that while AI tools provide easy access to information, the learning process can sometimes be less comprehensive.

% \emph{\textbf{"It encourages learning by guiding thought processes rather than just giving answers."-[P10]}}

% \emph{\textbf{"AI is helpful, but it can reduce our thinking power. We often rely on it rather than trying to solve the problem independently."-[P6]}}

% \subsubsection{\textbf{Participants' Perspective on Socratic Learning}}\hfill\\

% The Sakshm platform's approach to Socratic learning, particularly through its AI chatbot, Disha, elicits a range of opinions from users. Many appreciate the platform's method of providing hints rather than direct answers, as it encourages independent thinking and problem-solving. This method fosters a deeper understanding of coding concepts by allowing users to apply their logic and intuition to solve problems. Users have noted that Disha's hints help them think critically, especially when dealing with complex problems where a basic backbone is provided, nudging them in the right direction without spoon-feeding solutions. This approach is often likened to having an in-person tutor, guiding learners through a structured thought process.

% However, there needs to be more clarity on the effectiveness of this Socratic approach across different problem complexities. While many find it particularly useful for complex problems, where hints allow them to build intuition and approach problems methodically, some users express frustration when dealing with simpler queries or under time constraints. In such scenarios, they prefer direct answers for efficiency, indicating that while the Socratic method promotes learning, it can be perceived as less practical in time-sensitive situations. Users have suggested that an ideal AI integration in education would combine hints with the ability to evaluate a student's progress, offering snippets or sub-solutions when necessary, to strike a balance between fostering independent thinking and providing immediate assistance.

% Moreover, the distinction between answer-giving and Socratic learning models is highlighted. Users appreciate how Disha's approach aligns more closely with a Socratic tutor for harder questions, helping them build their solutions and thought processes. In contrast, for basic questions, users sometimes find direct answers more beneficial, especially when learning new concepts where step-by-step explanations are crucial for understanding. The consensus is that hints are preferable for learning, but during busy times or when under pressure, direct answers are more practical.

% \emph{\textbf{"The one that gives hints is better because it encourages us to think and doesn’t stop the thought process."-[P16]}}

% \emph{\textbf{"For hard questions, hints aren’t always enough, and sometimes I switch to ChatGPT for a full solution."-[P7]}}

% \subsubsection{\textbf{User Recommendations for Enhancement}}\hfill\\

% Users have recommended several enhancements to Sakshm to improve its effectiveness and engagement. They propose incorporating more advanced topics to bridge the gap between beginner and intermediate levels. A speech-to-text module has been suggested to aid interview preparation by simulating real-time coding scenarios. Enhancing the feedback mechanism with detailed insights on time complexity and providing test cases or follow-up exercises after explanations is also a priority. Improving the platform's user interface by reducing clutter and ensuring smooth navigation has been highlighted, along with integrating practical, real-world examples into exercises to enhance interest and applicability. Personalization remains a key focus, with users seeking adaptive features that cater to individual learning styles, offering tailored hints or solutions based on problem complexity. Additionally, fostering community and collaboration through features like discussion forums or peer review systems has been suggested to encourage peer-to-peer learning and engagement.


% \subsection{ Thematic analysis }
